ReRAW: RGB-to-RAW Image Reconstruction via Stratified Sampling for Efficient Object Detection on the Edge

Edge-based computer vision models running on compact, resource-limited devices benefit greatly from using unprocessed, detail-rich RAW sensor data instead of processed RGB images. Training these models, however, necessitates large labeled RAW datasets, which are costly and often impractical to obtain. Thus, converting existing labeled RGB datasets into sensor-specific RAW images becomes crucial for effective model training. In this paper, we introduce ReRAW, an RGB-to-RAW conversion model that achieves state-of-the-art reconstruction performance across five diverse RAW datasets. This is accomplished through ReRAW's novel multi-head architecture predicting RAW image candidates in gamma space. The performance is further boosted by a stratified sampling-based training data selection heuristic, which helps the model better reconstruct brighter RAW pixels. We finally demonstrate that pretraining compact models on a combination of high-quality synthetic RAW datasets (such as generated by ReRAW) and ground-truth RAW images for downstream tasks like object detection, outperforms both standard RGB pipelines, and RAW fine-tuning of RGB-pretrained models for the same task.

==> equations.tex <==
\begin{equation}
    ReRAW(\hat{I}_{\text{RGB}}, \hat{I}_{\text{F,RGB}}) = I_{\text{RAW}}
    \label{eq:eq1}
\end{equation}

\begin{equation}
    M(C(\hat{I}_{\text{RGB}}) * F(\hat{I}_{\text{F,RGB}}))=I_{i,RAW}, (i \in \{ 0, 1, \dots, n-1\})
    \label{eq:network-1}
\end{equation}

\begin{equation}
    G(\hat{I}_{\text{F,RGB}}) = \alpha_{i}, (i \in \{ 0, 1, \dots, n-1\}),  \sum_{i=0}^{n} \alpha_{i} = 1
    \label{eq:network-2}
\end{equation}

\begin{equation}
    \hat{I}_{i,RAW} = \hat{I}_{RAW}^{\gamma_{i}}, 
    \label{eq:network-3}
\end{equation}

\begin{equation}
    I_{RAW} = \sum_{i=0}^{n} I_{i,RAW}^{\frac{1}{\gamma_{i}}}*\alpha_{i}
    \label{eq:network-4}
\end{equation}

\begin{equation}
    \mathcal{L}_{ln}(\hat{I}, I) = \frac{-1}{CHW} \lvert(ln(1-|\hat{I}-I| + \epsilon)\rvert_{1}
    \label{eq:loss}
\end{equation}

\begin{equation}
    \mathcal{L} = \mathcal{L}_{ln}(\hat{I}_{RAW}, I_{RAW}) + \sum_{i=0}^{n} \mathcal{L}_{ln}(\hat{I}_{i,RAW}, I_{i,RAW}) 
    \label{eq:loss_g}
\end{equation}

\begin{equation}
    \hat{I}_{RAW}
    \hat{I}_{0,RAW}
    \hat{I}_{1,RAW}
    \hat{I}_{n-1,RAW}
\end{equation}
\begin{equation}
    I_{0,RAW}
    I_{1,RAW}
    I_{n-1,RAW}
\end{equation}
\begin{equation}
    \gamma_{0}
    \gamma_{1}
    \gamma_{n-1}
    \label{eq:eq-test}
\end{equation}

